LELANTE: LEveraging LLM for Automated ANdroid TEsting

Given natural language test case description for an Android application, existing testing approaches require developers to manually write scripts using tools such as Appium and Espresso to execute the corresponding test case. This process is labor-intensive and demands significant effort to maintain as UI interfaces evolve throughout development. In this work, we introduce LELANTE, a novel framework that utilizes large language models (LLMs) to automate test case execution without requiring pre-written scripts. LELANTE interprets natural language test case descriptions, iteratively generate action plans, and perform the actions directly on the Android screen using its GUI. LELANTE employs a screen refinement process to enhance LLM interpretability, constructs a structured prompt for LLMs, and implements an action generation mechanism based on chain-of-thought reasoning of LLMs. To further reduce computational cost and enhance scalability, LELANTE utilizes model distillation using a foundational LLM. In experiments across 390 test cases spanning 10 popular Android applications, LELANTE achieved a 73% test execution success rate. Our results demonstrate that LLMs can effectively bridge the gap between natural language test case description and automated execution, making mobile testing more scalable and adaptable.

==> sections/overview.tex <==
\section{Overview} \label{sec:over}

\textbf{\shortname{}} is an automated black-box testing framework \textit{(i.e., a testing approach where the internal workings of the application are unknown or inaccessible, and validation is performed solely based on inputs and observed outputs)} that utilizes \textbf{Large Language Models (LLMs)} and \textbf{Vision-Language Models (VLMs)} to execute and verify natural language test cases without requiring access to the application's source code. \shortname{} operates through a structured \textbf{two-stage pipeline}: first, it interprets and executes test cases through GUI interaction, and second, it verifies whether the application's state aligns with verification condition using a dual-layer validation mechanism. Figure~\ref{fig:LELANTE_architecture} illustrates the overall system architecture, which dynamically adapts to UI changes and ensures robust validation across diverse application states.

The \textbf{test case execution process} begins by processing natural language test instructions and refining the application's GUI representation into a structured format (\S\ref{sec:xml_to_html}). This step extracts relevant UI elements while filtering out unnecessary metadata to improve interpretability. The structured representation, combined with the test case and past actions, is then passed to an LLM, which generates a reasoning-driven sequence of actions to execute the test steps (\S\ref{sec:llm_reason}). The system iteratively interacts with the GUI, updating its understanding of the interface after each action (\S\ref{sec:action_grounding}), ensuring adaptability to dynamic UI elements. To optimize execution speed and reduce computational overhead, a smaller, task-specific model is distilled from a larger foundational LLM, preserving accuracy while enabling efficient real-time execution (\S\ref{sec:finetuning_test_ex}).

Following execution, the \textbf{verification process} evaluates whether the application's state aligns with the verification condition. The system first translates the test case into a structured verification condition (\S\ref{sec:verification_condition_generation}). A refined GUI representation is then extracted, preserving only relevant UI elements necessary for validation (\S\ref{sec:verification_xml_to_html}). An LLM-based reasoning process determines whether the observed UI state satisfies the verification condition (\S\ref{sec:verification_llm_reasoning}). Since some state changes involve graphical elements rather than textual descriptions, \shortname{} incorporates a vision-language model (VLM) to analyze screenshots and validate non-textual components such as icons and layout adjustments (\S\ref{sec:verification_vlm_integration}). Finally, to enable local, cost-effective verification, a distilled verification model is trained, leveraging knowledge distillation to retain high accuracy while reducing computational demands (\S\ref{sec:verification_model_distillation}). By integrating natural language processing, vision-based verification, and structured test execution, \shortname{} provides a fully automated, scalable approach to mobile application testing. The following sections explore each stage of the framework in detail.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/overall_pipeline.png}
    \caption{The high-level architecture of \shortname{}, illustrating the two-stage workflow.}
    \label{fig:LELANTE_architecture}
\end{figure}

